Discriminative Adversarial Privacy: Balancing Accuracy and Membership Privacy in Neural Networks

The remarkable proliferation of deep learning across various industries has underscored the importance of data privacy and security in AI pipelines. As the evolution of sophisticated Membership Inference Attacks (MIAs) threatens the secrecy of individual-specific information used for training deep learning models, Differential Privacy (DP) raises as one of the most utilized techniques to protect models against malicious attacks. However, despite its proven theoretical properties, DP can significantly hamper model performance and increase training time, turning its use impractical in real-world scenarios. Tackling this issue, we present Discriminative Adversarial Privacy (DAP), a novel learning technique designed to address the limitations of DP by achieving a balance between model performance, speed, and privacy. DAP relies on adversarial training based on a novel loss function able to minimise the prediction error while maximising the MIA's error. In addition, we introduce a novel metric named Accuracy Over Privacy (AOP) to capture the performance-privacy trade-off. Finally, to validate our claims, we compare DAP with diverse DP scenarios, providing an analysis of the results from performance, time, and privacy preservation perspectives.

==> tabs/aop1.tex <==
\begin{table}[!h]
    \caption{The AOP metric on the test sets ($\lambda=1$). Results improving the baseline are coloured in \textcolor{tabG}{green}, while results worse than the baseline are \textcolor{tabR}{red}. The best results among them are in \textbf{bold}, while the second best are \underline{underlined}.}
    \centering 
    \resizebox{\textwidth}{!}{%
    \begin{tabularx}{\textwidth}{| l || c | Y c Y Y Y Y Y |}
    \hline
      \textbf{Dataset} & \textbf{Baseline} & \textbf{Reg}  & \textbf{${\epsilon=0.5}$} & \textbf{${\epsilon=1}$}  & \textbf{${\epsilon=2}$}  & \textbf{${\epsilon=4}$}  & \textbf{DAP$_t$}  & \textbf{DAP$_v$}\\
    \hline \hline
    \textbf{Cifar-10} & 0.605 &	\textbf{\textcolor{tabG}{0.643}} &	\textcolor{tabR}{0.310} &	\textcolor{tabR}{0.355} & \textcolor{tabR}{0.402} & \textcolor{tabR}{0.415}	& \textcolor{tabG}{\underline{0.615}} &	\textcolor{tabG}{0.607}\\
    \textbf{Cifar-100} & 0.399	&\textbf{\textcolor{tabG}{0.428}}	&\textcolor{tabR}{0.039}	&\textcolor{tabR}{0.080}	&\textcolor{tabR}{0.089}	&\textcolor{tabR}{0.071}&	\textcolor{tabR}{\underline{0.305}}	& \textcolor{tabR}{0.273}\\
    \textbf{FMNIST} & 0.844	& \textcolor{tabR}{0.824} & \textcolor{tabR}{0.603}& \textcolor{tabR}{0.698}& \textcolor{tabR}{0.730} &	\textcolor{tabR}{0.766} &	\textcolor{tabG}{\underline{0.854}} & \textcolor{tabG}{\textbf{0.861}} \\
    \textbf{EuroSAT} & 0.880	& \textbf{\textcolor{tabG}{0.900}}	& \textcolor{tabR}{0.305}	& \textcolor{tabR}{0.586} &\textcolor{tabR}{0.681} & \textcolor{tabR}{0.643} 	& \textcolor{tabG}{\underline{0.898}} &	\textcolor{tabG}{0.891} \\
    \textbf{TinyImagenet} & 0.303 &	\textbf{\textcolor{tabG}{0.319}} &	\textcolor{tabR}{0.030} &	\textcolor{tabR}{0.032} &	\textcolor{tabR}{0.031} &	\textcolor{tabR}{0.025} &	\textcolor{tabR}{\underline{0.252}}& \textcolor{tabR}{0.213}\\
    \textbf{OxfordFlowers} & 0.372 & \textcolor{tabG}{\textbf{0.431}} &	\textcolor{tabR}{0.028} &	\textcolor{tabR}{0.047} &	\textcolor{tabR}{0.083} &	\textcolor{tabR}{0.131} &	\textcolor{tabR}{\underline{0.269}} &	\textcolor{tabR}{0.247} \\
    \textbf{STL-10} & 0.542 &	\textbf{\textcolor{tabG}{0.577}} &	\textcolor{tabR}{0.084} &	\textcolor{tabR}{0.135} & \textcolor{tabR}{0.247} & \textcolor{tabR}{0.288} &	\textcolor{tabR}{\underline{0.472}}& \textcolor{tabR}{0.379} \\
    \textbf{Cinic-10} & 0.588 & \textcolor{tabR}{\underline{0.577}} & \textcolor{tabR}{0.279} &	\textcolor{tabR}{0.339} & \textcolor{tabR}{0.389} &	\textcolor{tabR}{0.402} &	\textcolor{tabR}{0.565}	& \textcolor{tabR}{\textbf{0.578}}\\
    \hline
    \textbf{Average} & 0.567 & \textbf{\textcolor{tabG}{0.587}} & \textcolor{tabR}{0.210} &	\textcolor{tabR}{0.284} &	\textcolor{tabR}{0.331} & \textcolor{tabR}{0.343}  & \textcolor{tabR}{\underline{0.529}} & \textcolor{tabR}{0.506}\\
    \hline
    \end{tabularx}}%
    \label{table:aop1}
\end{table}

==> tabs/aop10.tex <==
\begin{table}[!h]
    \caption{The AOP metric on the test sets ($\lambda=10$). Results improving the baseline are coloured in \textcolor{tabG}{green}, while results worse than the baseline are \textcolor{tabR}{red}. The best results among them are in \textbf{bold}, while the second best are \underline{underlined}.}
    \centering 
    \resizebox{\textwidth}{!}{%
    \begin{tabularx}{\textwidth}{| l || c | Y c Y Y Y Y Y |}
    \hline
      \textbf{Dataset} & \textbf{Baseline} & \textbf{Reg}  & \textbf{${\epsilon=0.5}$} & \textbf{${\epsilon=1}$}  & \textbf{${\epsilon=2}$}  & \textbf{${\epsilon=4}$}  & \textbf{DAP$_t$}  & \textbf{DAP$_v$}\\
    \hline \hline
    \textbf{Cifar-10} & 0.059 &	\textcolor{tabG}{0.079} &	\textcolor{tabG}{0.283} &	\textcolor{tabG}{0.225} & \textcolor{tabG}{0.287} & \textcolor{tabG}{0.394}	& \textcolor{tabG}{\underline{0.543}} &	\textcolor{tabG}{\textbf{0.555}}\\
    \textbf{Cifar-100} & 0.074	& \textcolor{tabR}{0.061}	&\textcolor{tabR}{0.039}	&\textcolor{tabR}{0.062}	&\textcolor{tabG}{0.078}	&\textcolor{tabR}{0.064}&	\textcolor{tabG}{\underline{0.230}}	& \textcolor{tabG}{\textbf{0.245}}\\
    \textbf{FMNIST} & 0.346	& \textcolor{tabR}{0.288} & \textcolor{tabG}{0.581}& \textcolor{tabG}{0.674}& \textcolor{tabG}{0.680} &	\textcolor{tabG}{0.701} &	\textcolor{tabG}{\underline{0.754}} & \textcolor{tabG}{\textbf{0.773}} \\
    \textbf{EuroSAT} & 0.412	& \textcolor{tabG}{0.551}	& \textcolor{tabR}{0.279}	& \textcolor{tabG}{0.565} &\textcolor{tabG}{0.681} & \textcolor{tabG}{0.621} 	& \textcolor{tabG}{\underline{0.882}} &	\textcolor{tabG}{\textbf{0.875}} \\
    \textbf{TinyImagenet} & 0.056 &	\textcolor{tabG}{0.069} &	\textcolor{tabR}{0.023} &	\textcolor{tabR}{0.031} &	\textcolor{tabR}{0.021} &	\textcolor{tabR}{0.023} &	\textcolor{tabG}{\textbf{0.190}}& \textcolor{tabG}{\underline{0.181}}\\
    \textbf{OxfordFlowers} & 0.008 & \textcolor{tabG}{0.009} &	\textcolor{tabG}{0.014} &	\textcolor{tabG}{0.025} &	\textcolor{tabG}{0.052} &	\textcolor{tabG}{0.075} &	\textcolor{tabG}{\underline{0.269}} &	\textcolor{tabG}{\textbf{0.247}} \\
    \textbf{STL-10} & 0.099 &	\textcolor{tabG}{0.198} &	\textcolor{tabR}{0.081} &	\textcolor{tabR}{0.089} & \textcolor{tabG}{0.226} & \textcolor{tabG}{0.283} &	\textcolor{tabG}{\textbf{0.409}}& \textcolor{tabG}{\underline{0.341}} \\
    \textbf{Cinic-10} & 0.175 & \textcolor{tabR}{0.091} & \textcolor{tabG}{0.274} &	\textcolor{tabG}{0.321} & \textcolor{tabG}{0.368} &	\textcolor{tabG}{0.374} &	\textcolor{tabG}{\underline{0.464}}	& \textcolor{tabG}{\textbf{0.510}}\\
    \hline
    \textbf{Average} & 0.154 & \textcolor{tabG}{0.168} & \textcolor{tabG}{0.197} &	\textcolor{tabG}{0.249} &	\textcolor{tabG}{0.299} & \textcolor{tabG}{0.317}  & \textcolor{tabG}{\underline{0.451}} & \textcolor{tabG}{\textbf{0.456}}\\
    \hline
    \end{tabularx}}%
    \label{table:aop10}
    % \vspace{-10pt}
\end{table}

==> tabs/aop5.tex <==
\begin{table}[!h]
    \caption{The AOP metric on the test sets ($\lambda=5$). Results improving the baseline are coloured in \textcolor{tabG}{green}, while results worse than the baseline are \textcolor{tabR}{red}. The best results among them are in \textbf{bold}, while the second best are \underline{underlined}.}
    \centering 
    \resizebox{\textwidth}{!}{%
    \begin{tabularx}{\textwidth}{| l || c | Y c Y Y Y Y Y |}
    \hline
      \textbf{Dataset} & \textbf{Baseline} & \textbf{Reg}  & \textbf{${\epsilon=0.5}$} & \textbf{${\epsilon=1}$}  & \textbf{${\epsilon=2}$}  & \textbf{${\epsilon=4}$}  & \textbf{DAP$_t$}  & \textbf{DAP$_v$}\\
    \hline \hline
    \textbf{Cifar-10} & 0.214 &	\textcolor{tabG}{0.253} &	\textcolor{tabG}{0.298} &	\textcolor{tabG}{0.290} & \textcolor{tabG}{0.346} & \textcolor{tabG}{0.406}	& \textcolor{tabG}{\underline{0.582}} &	\textcolor{tabG}{\textbf{0.583}}\\
    \textbf{Cifar-100} & 0.188	& \textcolor{tabR}{0.180}	&\textcolor{tabR}{0.039}	&\textcolor{tabR}{0.072}	&\textcolor{tabR}{0.084}	&\textcolor{tabR}{0.068}&	\textcolor{tabG}{\textbf{0.269}}	& \textcolor{tabG}{\underline{0.260}}\\
    \textbf{FMNIST} & 0.568	& \textcolor{tabR}{0.516} & \textcolor{tabG}{0.593}& \textcolor{tabG}{0.687}& \textcolor{tabG}{0.707} &	\textcolor{tabG}{0.736} &	\textcolor{tabG}{\underline{0.808}} & \textcolor{tabG}{\textbf{0.821}} \\
    \textbf{EuroSAT} & 0.629	& \textcolor{tabG}{0.723}	& \textcolor{tabR}{0.293}	& \textcolor{tabR}{0.276} &\textcolor{tabG}{0.681} & \textcolor{tabG}{0.633} 	& \textbf{\textcolor{tabG}{0.891}} &	\textcolor{tabG}{\underline{0.884}} \\
    \textbf{TinyImagenet} & 0.143 &	\textcolor{tabG}{0.162} &	\textcolor{tabR}{0.027} &	\textcolor{tabR}{0.032} &	\textcolor{tabR}{0.026} &	\textcolor{tabR}{0.024} &	\textcolor{tabG}{\textbf{0.222}}& \textcolor{tabG}{\underline{0.198}}\\
    \textbf{OxfordFlowers} & 0.069 & \textcolor{tabG}{0.079} &	\textcolor{tabR}{0.020} &	\textcolor{tabR}{0.036} &	\textcolor{tabR}{0.067} &	\textcolor{tabG}{0.102} &	\textcolor{tabG}{\underline{0.201}} &	\textbf{\textcolor{tabG}{0.209}} \\
    \textbf{STL-10} & 0.255 &	\textcolor{tabG}{0.359} &	\textcolor{tabR}{0.082} &	\textcolor{tabR}{0.112} & \textcolor{tabR}{0.238} & \textcolor{tabG}{0.286} &	\textcolor{tabG}{\textbf{0.443}}& \textcolor{tabR}{\underline{0.362}} \\
    \textbf{Cinic-10} & 0.343 & \textcolor{tabR}{0.254} & \textcolor{tabR}{0.277} &	\textcolor{tabR}{0.331} & \textcolor{tabG}{0.379} &	\textcolor{tabG}{0.389} &	\textcolor{tabG}{\underline{0.517}}	& \textcolor{tabG}{\textbf{0.547}}\\
    \hline
    \textbf{Average} & 0.301 & \textcolor{tabG}{0.316} & \textcolor{tabR}{0.204} &	\textcolor{tabR}{0.267} &	\textcolor{tabG}{0.316} & \textcolor{tabG}{0.331}  & \textbf{\textcolor{tabG}{0.492}} & \textcolor{tabG}{\underline{0.483}}\\
    \hline
    \end{tabularx}}%
    \label{table:aop5}
\end{table}

==> tabs/aucmiss.tex <==
\begin{table}[!h]
    \caption{The AUC metric of the MIAs over the wrongly classified samples. Results improving the baseline are coloured in \textcolor{tabG}{green}, while results worse than the baseline are \textcolor{tabR}{red}. The best results among them are in \textbf{bold}, while the second best are \underline{underlined}.}
    \centering 
    \resizebox{\textwidth}{!}{%
    \begin{tabularx}{\textwidth}{| l || c | Y c Y Y Y Y Y |}
    \hline
    \textbf{Dataset} & \textbf{Baseline} & \textbf{Reg}  & \textbf{${\epsilon=0.5}$} & \textbf{${\epsilon=1}$}  & \textbf{${\epsilon=2}$}  & \textbf{${\epsilon=4}$}  & \textbf{DAP$_t$}  & \textbf{DAP$_v$}\\
    \hline \hline
    \textbf{Cifar-10} & 0.753 & \textcolor{tabG}{0.689} & \underline{\textcolor{tabG}{0.505}} & \textbf{\textcolor{tabG}{0.503}} & \textbf{\textcolor{tabG}{0.503}} & \textcolor{tabG}{0.506} & \textcolor{tabG}{0.510} & \underline{\textcolor{tabG}{0.505}}\\
    \textbf{Cifar-100} & 0.610 & \textcolor{tabR}{0.627} & \textbf{\textcolor{tabG}{0.501}} & \textcolor{tabG}{0.506} & \textcolor{tabG}{0.538} & \underline{\textcolor{tabG}{0.505}} & \textcolor{tabG}{0.518} & \textcolor{tabG}{0.509}\\
    \textbf{FMNIST} & 0.659 & \textcolor{tabR}{0.768} & \underline{\textcolor{tabG}{0.502}} & \textcolor{tabG}{0.506} & \underline{\textcolor{tabG}{0.502}} & \textbf{\textcolor{tabG}{0.500}} & \textcolor{tabG}{0.523} & \textcolor{tabG}{0.527} \\
    \textbf{EuroSAT} & 0.698 & \textcolor{tabG}{0.563} & \textbf{\textcolor{tabG}{0.500}} & \underline{\textcolor{tabG}{0.501}} & \textcolor{tabG}{0.523} & \textcolor{tabG}{0.504} & \textcolor{tabG}{0.527} & \textcolor{tabG}{0.528}\\
    \textbf{TinyImagenet} & 0.585 & \textcolor{tabG}{0.565} & \textcolor{tabG}{0.504} & \underline{\textcolor{tabG}{0.502}} & \textbf{\textcolor{tabG}{0.501}} & \textcolor{tabG}{0.505} & \textcolor{tabG}{0.518} & \textcolor{tabG}{0.508}\\
    \textbf{OxfordFlowers} & 0.785 & \textcolor{tabR}{0.837} & \underline{\textcolor{tabG}{0.529}} & \textcolor{tabG}{0.555} & \textbf{\textcolor{tabG}{0.518}} & \textcolor{tabG}{0.532} & \textcolor{tabG}{0.547} & \textcolor{tabG}{0.537}\\
    \textbf{STL-10} & 0.636 & \textcolor{tabG}{0.567} & \textbf{\textcolor{tabG}{0.500}} & \textcolor{tabG}{0.506} & \textcolor{tabG}{0.506} & \underline{\textcolor{tabG}{0.504}} & \textcolor{tabG}{0.509} & \underline{\textcolor{tabG}{0.504}}\\
    \textbf{Cinic-10} & 0.560 & \textcolor{tabR}{0.649} & \textbf{\textcolor{tabG}{0.501}} & \textcolor{tabG}{0.503} & \textcolor{tabG}{0.503} & \underline{\textcolor{tabG}{0.502}} & \textcolor{tabG}{0.508} & \textcolor{tabG}{0.510}\\
    \hline
    \textbf{Average} & 0.661 & \textcolor{tabG}{0.658} & \textbf{\textcolor{tabG}{0.505}} & \textcolor{tabG}{0.510} & \textcolor{tabG}{0.512} & \textcolor{tabG}{\underline{0.507}} & \textcolor{tabG}{0.520} & \textcolor{tabG}{0.516}\\
    \hline
    \end{tabularx}}%
    \label{table:miss}
\end{table}


==> tabs/aucok.tex <==
\begin{table}[!h]
    \caption{The AUC metric of the MIAs over the correctly classified samples. Results improving the baseline are coloured in \textcolor{tabG}{green}, while results worse than the baseline are \textcolor{tabR}{red}. The best results among them are in \textbf{bold}, while the second best are \underline{underlined}.}
    \centering 
    \resizebox{\textwidth}{!}{%
    \begin{tabularx}{\textwidth}{| l || c | Y c Y Y Y Y Y |}
    \hline
    \textbf{Dataset} & \textbf{Baseline} & \textbf{Reg}  & \textbf{$\epsilon=0.5$} & \textbf{$\epsilon=1$}  & \textbf{ $\epsilon=2$}  & \textbf{$\epsilon=4$}  & \textbf{DAP$_t$}  & \textbf{DAP$_v$}\\
    \hline \hline
    \textbf{Cifar-10} & 0.545 & \textcolor{tabG}{0.537} & \textbf{\textcolor{tabG}{0.500}} & \textcolor{tabG}{\underline{0.502}} & \textcolor{tabG}{0.503} & \textcolor{tabG}{0.506} & \textcolor{tabG}{0.507} & \textcolor{tabG}{0.504} \\
    \textbf{Cifar-100} & 0.516 & \textcolor{tabR}{0.517} & \textcolor{tabG}{0.512} & \textcolor{tabR}{0.521} & \textcolor{tabG}{\underline{0.508}} & \textcolor{tabG}{0.511} & \textbf{\textcolor{tabG}{0.507}} & \textcolor{tabG}{0.509}\\
    \textbf{FMNIST} & 0.514 & \textcolor{tabR}{0.532} & \textcolor{tabG}{\underline{0.504}} & \textcolor{tabG}{0.505} & \textcolor{tabG}{0.511} & \textcolor{tabG}{0.510} & \textcolor{tabG}{0.505} & \textbf{\textcolor{tabG}{0.501}} \\
    \textbf{EuroSAT} & 0.514 & \textcolor{tabG}{\underline{0.503}} & \textcolor{tabR}{0.516} & \textcolor{tabG}{0.508} & \textcolor{tabG}{0.508} & \textcolor{tabR}{0.532} & \textbf{\textcolor{tabG}{0.502}} & \textbf{\textcolor{tabG}{0.502}}\\
    \textbf{TinyImagenet} & 0.509 & \textcolor{tabG}{0.506} & \textcolor{tabG}{0.504} & \textcolor{tabR}{0.530} & \textcolor{tabR}{0.544} & \textcolor{tabR}{0.520} & \textcolor{tabG}{\underline{0.502}} & \textbf{\textcolor{tabG}{0.501}} \\
    \textbf{OxfordFlowers} & 0.556 & \textcolor{tabR}{0.595} & \textcolor{tabR}{0.877} & \textcolor{tabR}{0.677} & \textcolor{tabR}{0.589} & \textcolor{tabR}{0.590} & \textbf{\textcolor{tabG}{0.529}} & \textcolor{tabG}{\underline{0.535}}\\
    \textbf{STL-10} & 0.522 & \textcolor{tabG}{0.508} & \textcolor{tabG}{0.521} & \textcolor{tabG}{0.513} & \textbf{\textcolor{tabG}{0.501}} & \textcolor{tabG}{0.505} & \textcolor{tabG}{\underline{0.503}} & \textcolor{tabG}{0.504}\\
    \textbf{Cinic-10} & 0.508 & \textcolor{tabR}{0.534} & \textcolor{tabG}{\underline{0.505}} & \textbf{\textcolor{tabG}{0.501}} & \textbf{\textcolor{tabG}{0.501}} & \textbf{\textcolor{tabG}{0.501}} & \textbf{\textcolor{tabG}{0.501}} & \textbf{\textcolor{tabG}{0.501}}\\
    \hline
    \textbf{Average} & 0.523 & \textcolor{tabR}{0.529} & \textcolor{tabR}{0.555} & \textcolor{tabR}{0.532} & \textcolor{tabG}{\underline{0.521}} & \textcolor{tabG}{0.522} & \textbf{\textcolor{tabG}{0.507}} & \textbf{\textcolor{tabG}{0.507}}\\
    \hline
    \end{tabularx}}%
    \label{table:ok}
\end{table}

==> tabs/time.tex <==
\begin{table}[!h]
    \caption{The training time (seconds) of the experiments performed compared to the Baseline. Results improving it are coloured in \textcolor{tabG}{green}, while those worsen it in \textcolor{tabR}{red}. The best results are in \textbf{bold} and the second best are \underline{underlined}.}
    \centering 
    \resizebox{\textwidth}{!}{%
    \begin{tabularx}{\textwidth}{| l || c | Y c Y Y Y Y Y |}
    \hline
      \textbf{Dataset} & \textbf{Baseline} & \textbf{Reg}  & \textbf{$\epsilon=0.5$} & \textbf{$\epsilon=1$}  & \textbf{ $\epsilon=2$}  & \textbf{$\epsilon=4$}  & \textbf{DAP$_t$}  & \textbf{DAP$_v$}\\
    \hline \hline
    \textbf{Cifar-10} & 492 & \textcolor{tabR}{\underline{888}} & \textcolor{tabG}{\textbf{456}} & \textcolor{tabR}{3646} & \textcolor{tabR}{13379} & \textcolor{tabR}{47392} & \textcolor{tabR}{4190} & \textcolor{tabR}{4656}  \\
    \textbf{Cifar-100} & 1596 & \textcolor{tabR}{\underline{2386}} & \textcolor{tabG}{\textbf{427}} & \textcolor{tabR}{3458} & \textcolor{tabR}{12583} & \textcolor{tabR}{44174} & \textcolor{tabR}{5881} & \textcolor{tabR}{4069}\\
    \textbf{FMNIST} & 400 & \textcolor{tabR}{\textbf{826}} & \textcolor{tabR}{\underline{850}} & \textcolor{tabR}{5396} & \textcolor{tabR}{17265} & \textcolor{tabR}{51916} & \textcolor{tabR}{2874} & \textcolor{tabR}{3800} \\
    \textbf{EuroSAT} & 395 & \textcolor{tabG}{\underline{359}} & \textcolor{tabG}{\textbf{72}} & \textcolor{tabR}{2409} & \textcolor{tabR}{8996} & \textcolor{tabR}{31485} & \textcolor{tabR}{1496} & \textcolor{tabR}{2681} \\
    \textbf{TinyImagenet} & 3913 & \textcolor{tabG}{\textbf{2140}} & \textcolor{tabR}{\underline{11082}} & \textcolor{tabR}{55123} & \textcolor{tabR}{194238} & \textcolor{tabR}{329391} & \textcolor{tabR}{21140} & \textcolor{tabR}{14105}\\
    \textbf{OxfordFlowers} & 80 & \textcolor{tabR}{168} & \textcolor{tabG}{\textbf{23}} & \textcolor{tabR}{171} & \textcolor{tabR}{765} & \textcolor{tabR}{2793} & \textcolor{tabR}{1158} & \textcolor{tabR}{739} \\
    \textbf{STL-10} & 104 & \textcolor{tabR}{172} & \textcolor{tabG}{\textbf{38}} & \textcolor{tabR}{182} & \textcolor{tabR}{978} & \textcolor{tabR}{3585} & \textcolor{tabR}{1559} & \textcolor{tabR}{386} \\
    \textbf{Cinic-10} & \textbf{2630} & \textcolor{tabR}{\underline{3530}} & \textcolor{tabR}{3929} & \textcolor{tabR}{19477} & \textcolor{tabR}{69790} & \textcolor{tabR}{116314} & \textcolor{tabR}{21034} & \textcolor{tabR}{21124}\\
    \hline
    \textbf{Average} & \textbf{1201.2} & \textcolor{tabR}{\underline{1308.6}} & \textcolor{tabR}{2109.6} & \textcolor{tabR}{11232.8} & \textcolor{tabR}{39749.3} & \textcolor{tabR}{78381.2} & \textcolor{tabR}{7416.5} & \textcolor{tabR}{6445}\\
    \hline
    \end{tabularx}}%
    \label{table:time}
\end{table}
